DANLIP: Deep Autoregressive Networks for Locally Interpretable Probabilistic Forecasting

Despite the high performance of neural network-based time series forecasting methods, the inherent challenge in explaining their predictions has limited their applicability in certain application areas. Due to the difficulty in identifying causal relationships between the input and output of such black-box methods, they rarely have been adopted in domains such as legal and medical fields in which the reliability and interpretability of the results can be essential. In this paper, we propose \model, a novel deep learning-based probabilistic time series forecasting architecture that is intrinsically interpretable. We conduct experiments with multiple datasets and performance metrics and empirically show that our model is not only interpretable but also provides comparable performance to state-of-the-art probabilistic time series forecasting methods. Furthermore, we demonstrate that interpreting the parameters of the stochastic processes of interest can provide useful insights into several application areas.

==> other_files/Defs.tex <==

\usepackage{xcolor}
\usepackage{color}

%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage[noend]{algpseudocode}
%\usepackage[]{algorithm2e}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}


% TABLE RELATED (JUYOUNG)
\usepackage{tabularx}
\newcolumntype{s}{>{\hsize=.32\hsize}X}
\usepackage{longtable,tabularx,ltxtable}
\usepackage{ragged2e}  % for \RaggedRight and \Centering macros
\newcolumntype{L}{>{\RaggedRight\arraybackslash}X}
\usepackage{supertabular}

\usepackage{enumitem}

% \usepackage[driverfallback=dvipdfm]{hyperref}%backref,

% ESTHETICS (JUYOUNG)
\PassOptionsToPackage{hyphens}{url}

%\usepackage{cite}
\usepackage{multirow}
% \setlength\parindent{0pt}
% Set the typeface to Times Roman

\usepackage{comment}

\usepackage{tikz,tikz-3dplot,graphicx} %,pgfplots,animate,pstricks,epsfig}
\usetikzlibrary{arrows,shadings,shadows,automata,shapes,calc,positioning,patterns,decorations.markings,decorations.pathmorphing,plotmarks,angles,backgrounds,fit}

% Custom params
\usepackage{amsmath, amsthm, amsfonts, amssymb, bm}

\newtheorem*{df}{Definition}
% EXTRA PACKAGES
% \usepackage{subfig}
\usepackage{float}
\usepackage{url}
%\usepackage{enumerate}
\usepackage{color}   %May be necessary if you want to color links

% TIKZ PACK
\usepackage{tikz}
\usepackage{mathdots}
\usepackage{yhmath}
\usepackage{cancel}
\usepackage{color}
\usepackage{siunitx}
\usepackage{array}
\usepackage{multirow}
% \usepackage{amssymb}
\usepackage{gensymb}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage[demo]{rotating}
\usetikzlibrary{fadings}
\usetikzlibrary{patterns}
\usetikzlibrary{shadows.blur}
\usepackage{times}
\usepackage{mathtools, cuted}
\usepackage{geometry}

% \usepackage{url}


\usetikzlibrary{fadings}
\usetikzlibrary{patterns}
\usetikzlibrary{shadows.blur}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% TIKZ PACK
\usepackage{tikz}
\usepackage{mathdots}
\usepackage{yhmath}
\usepackage{cancel}
\usepackage{color}
\usepackage{siunitx}
\usepackage{array}
\usepackage{multirow}
\usepackage{amssymb}
\usepackage{gensymb}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage[demo]{rotating}


%% The graphicx package provides the includegraphics command.
\usepackage{graphicx}
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Custom params
\usepackage{amsmath, amsthm, amsfonts,amssymb, bm}
\usepackage{svg}
% EXTRA PACKAGES
\usepackage{subfig}
\usepackage{float}
\usepackage{url}
\usepackage{enumerate}
\usepackage{color}   %May be necessary if you want to color links
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true, %set true if you want colored links
%     linktoc=all,     %set to all if you want both sections and subsections linked
%     linkcolor=blue,  %choose some color if you want links to stand out
% }
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{bm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cred}{\color{red!85!black}}


% SPRINGER: 
% \setlength{\rotFPtop}{0pt plus 1fil}% <- add this line after loading rotating
% \setlength{\rotFPbot}{0pt plus 1fil}% <- maybe its better to add this line too

% \usepackage[colorlinks = true,
%              linkcolor = blue,
%              urlcolor  = blue,
%              citecolor = blue,
%              anchorcolor = blue]{hyperref}
\usepackage{cite}
\usepackage{tabularx}

% \def\@seccntformat#1{\@ifundefined{#1@cntformat}%
%   {\csname the#1\endcsname\quad}  % default
%   {\csname #1@cntformat\endcsname}% enable individual control
% }
% \let\oldappendix\appendix %% save current definition of \appendix
% \renewcommand\appendix{%
%     \oldappendix
%     \newcommand{\section@cntformat}{\appendixname~\thesection\quad}
% }

==> other_files/notations.tex <==
\begin{table}[htp]
\small
\begin{tabularx}{\textwidth}{lX}
\toprule
% SETS
\textbf{\textsc{Sets:}} \\
$\parSetOrgans$ & Set of OARs, $\indTissue \in \parSetOrgans$ \\
$\parSetTumors$ & Set of tumors, $\indTumor \in \parSetTumors$ \\
$\parSetBeamlets$ & Set of beamlets, $\indBeamlet \in \parSetBeamlets$\\
$\parSetTissues = \parSetOrgans \cup \parSetTumors$ & Set of tissues, $\indTissue \in \parSetTissues$\\
$\parSetVoxels$ & Set of voxels of $\indTissue \in \parSetTissues$, $\indVoxel \in \parSetVoxels$ \\*[0.05cm] 
\midrule
\midrule
% PARAMETERS
\textbf{\textsc{Parameters:}} \\
\textit{Deterministic:} \\
$\parFraction$ & Total number of fractions \\
$\parMaxDose$ & Maximum dose allowed for voxel $\indVoxel \in \parSetVoxels$ of tissue $\indTissue \in \parSetTissues$  \\
$\parMinDose$ & Minimum dose required for voxel $\indVoxel \in \parSetVoxels$ of tissue $\indTissue \in \parSetTissues$   \\
$\alpha_{\indTissue}^+$ & Overdose minimization weight for tissue $\indTissue \in \parSetTissues$   \\
$\alpha_{\indTumor}^+$ & Overdose minimization weight for tumor  \\ 
$\parMaxDoseFractionwise$ & Maximum dose allowed for voxel $\indVoxel \in \parSetVoxels$ of tissue $\indTissue \in \parSetTissues$, at fraction $f \in [\parFraction]$  \\
$\parMinDoseFractionwise$ & Minimum dose required for voxel $\indVoxel \in \parSetVoxels$ of tissue $\indTissue \in \parSetTissues$, at fraction $f \in [\parFraction]$  \\
$\parOverdoseFractionwiseConstant$ & Overdose penalty weight for tissue $\indTissue \in \parSetTissues$ for fraction $\indFraction \in [\parFraction]$  \\
$\parUnderdoseFractionwiseConstant$ & Overdose penalty weight for tumor $\indTumor \in \parSetTumors$ for fraction $\indFraction \in [\parFraction]$\\*[0.05cm] 
\midrule
\textit{Uncertain:}  \\ 
$\parDoseMatrix$ & Dose received by voxel $\indVoxel \in \parSetVoxels$ of tissue $l \in \parSetTissues$ when unit beam is shot through $\indBeamlet \in \parSetBeamlets$ \\*[0.05cm] 
\midrule
\midrule
% DECISION VARIABLES
\textbf{\textsc{Decisions:}} \\*[0.1cm]
$\varIrradiationTime$ &  Intensity of beam to shoot through beamlet $\indBeamlet \in \parSetBeamlets$ at the end of fraction $\indFraction \in [\parFraction]$  \\
$\varDeliveredDose$ & Dose received by voxel $\indVoxel \in \parSetVoxels$ at the end of fraction $\indFraction \in [\parFraction]$  \\
$\varEOHOver$ &  Penalty of overdosing voxel $\indVoxel \in \parSetVoxels$ of structure $\indTissue \in \parSetTissues$ at the end of of all treatment plan  \\
$\varEOHUnder$ &  Penalty of underdosing voxel $\indVoxel \in \parSetVoxels$ of structure $\indTissue \in \parSetTissues$ at the end of of all treatment plan   \\
$\varOver$ &  Penalty of overdosing voxel $\indVoxel \in \parSetVoxels$ of structure $\indTissue \in \parSetTissues$ at the end of fraction $\indFraction \in [\parFraction]$   \\ 
$\varUnder$ &  Penalty of underdosing voxel $\indVoxel \in \parSetVoxels$ of structure $\indTissue \in \parSetTissues$ at the end of fraction $\indFraction \in [\parFraction]$ \\
$\varInventory$ &  Cumulative amount of dose received at the beginning of fraction $\indFraction \in [\parFraction+1]$   \\*[0.15cm]
\bottomrule
\hline
\end{tabularx}
\caption{Notation used in the fractionated multistage stochastic IMRT planning model}
\label{tab:MSPIMRTnotations}
\end{table}





==> tables/results.tex <==
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
%                 & \multicolumn{4}{c|}{\textbf{Rossmann Dataset}}                             & \multicolumn{4}{c|}{\textbf{Ohio Dataset}}                                 \\ \hline
%                 & \textbf{NRMSE} & \textbf{0.3-risk} & \textbf{0.5-risk} & \textbf{0.9-risk} & \textbf{NRMSE} & \textbf{0.3-risk} & \textbf{0.5-risk} & \textbf{0.9-risk} \\ \hline
% \textbf{DeepAR} & 0.39           & 0.18              & 0.09              & 0.40              & 0.14               & 0.47                  & 0.10                  & 0.49                  \\ \hline
% \textbf{Ours}   & 0.25           & 0.21              & 0.06              & 0.14              & 0.15           & 0.45              & 0.08              & 0.49              \\ \hline
% \end{tabular}
% \begin{tabular}{ll|ll}
%                                                         &                   & \textbf{DeepAR} & \textbf{POLAR} \\ \hline
% \multicolumn{1}{l|}{\multirow{4}{*}{\textbf{Rossmann}}} & \textbf{NRMSE}    & 0.39            & 0.25           \\
% \multicolumn{1}{l|}{}                                   & \textbf{0.3-risk} & 0.18            & 0.21           \\
% \multicolumn{1}{l|}{}                                   & \textbf{0.5-risk} & 0.09            & 0.06           \\
% \multicolumn{1}{l|}{}                                   & \textbf{0.9-risk} & 0.40            & 0.14           
% \end{tabular}
\begin{tabular}{ll|ll}
                                      &                   & \textbf{DeepAR} & \textbf{ITS} \\ \hline
\multirow{3}{*}{\textbf{Electricity}} & \textbf{ND}       & 0.528           & 0.481        \\
                                      & \textbf{0.5-risk} & 0.399           & 0.405        \\
                                      & \textbf{0.9-risk} & 0.212           & 0.218        \\ \hline
\multirow{3}{*}{\textbf{Rossmann}}    & \textbf{ND}       & 0.388           & 0.399        \\
                                      & \textbf{0.5-risk} & 0.192           & 0.202        \\
                                      & \textbf{0.9-risk} & 0.100           & 0.185       
\end{tabular}
% \begin{tabular}{ll|ll}
%                                       &                   & \textbf{DeepAR} & \textbf{ITS} \\ \hline
% \multirow{3}{*}{\textbf{Electricity}} & \textbf{ND}       & 0.528           & 0.481        \\
%                                       & \textbf{0.5-risk} & 0.399           & 0.405        \\
%                                       & \textbf{0.9-risk} & 0.212           & 0.218        \\ \hline
% \multirow{3}{*}{\textbf{Rossmann}}    & \textbf{ND}       & 0.388           & 0.1856        \\
%                                       & \textbf{0.5-risk} & 0.192           & 0.0012        \\
%                                       & \textbf{0.9-risk} & 0.100           & 0.0016       
% \end{tabular}
